Zorua: Enhancing Programming Ease, Portability, and Performance in GPUs by Decoupling Programming Models from Resource Management

The application resource specification--a static specification of several parameters such as the number of threads and the scratchpad memory usage per thread block--forms a critical component of the existing GPU programming models. This specification determines the performance of the application during execution because the corresponding on-chip hardware resources are allocated and managed purely based on this specification. This tight coupling between the software-provided resource specification and resource management in hardware leads to significant challenges in programming ease, portability, and performance, as we demonstrate in this work. Our goal in this work is to reduce the dependence of performance on the software-provided resource specification to simultaneously alleviate the above challenges. To this end, we introduce Zorua, a new resource virtualization framework, that decouples the programmer-specified resource usage of a GPU application from the actual allocation in the on-chip hardware resources. Zorua enables this decoupling by virtualizing each resource transparently to the programmer. We demonstrate that by providing the illusion of more resources than physically available, Zorua offers several important benefits: (i) Programming Ease: Zorua eases the burden on the programmer to provide code that is tuned to efficiently utilize the physically available on-chip resources. (ii) Portability: Zorua alleviates the necessity of re-tuning an application's resource usage when porting the application across GPU generations. (iii) Performance: By dynamically allocating resources and carefully oversubscribing them when necessary, Zorua improves or retains the performance of applications that are already highly tuned to best utilize the resources. The holistic virtualization provided by Zorua has many other potential uses which we describe in this paper.

==> sections/approach.tex <==
There are two key challenges that need to be addressed in effectively
virtualizing multiple on-chip
resources. We now discuss these challenges
and provide an overview of how we address them.

\subsection{Challenges in Virtualization}
\label{sec:virt-challenges}
\textbf{Challenge 1:}\emph{ Controlling the Extent of Oversubscription.} A key challenge is to determine the \emph{extent} of oversubscription or the
size of the virtual space for each resource. Increasing the oversubscription enables more parallelism and performance. However, this is a
tradeoff because of the overhead of spilling resources to the swap
space. 
%Overly oversubscribing any resource would exacerbate the overheads and
%destroy the benefits of parallelism.  
This tradeoff is especially challenging because of the variation in resource
requirements at runtime. As a result, the size of the
virtual space for each resource needs to be continuously tuned to make the
tradeoff between more parallelism and less overhead. 

\textbf{Challenge 2:} \emph{Control and Coordination for Multiple
Resources.} Once we have determined the size of each of the virtual resources, a key
challenge is to efficiently map the constantly varying virtual resource space to the
available physical resources and its swap space. 
%The virtual space provides
%the illusion of more resources than the physical space by employing the swap
%space. However, at any given time it is of vital importance to control the
%mapping of resources to the physical and swap space. 
This is important for two reasons. First, it is
critical to minimize accesses to the swap space. Accessing the swap space for
the register file or scratchpad involves potentially expensive accesses to
global memory. In the case of
threads, only those mapped to the physical space are available for scheduling. Second, each thread requires multiple resources for execution,
each of which may be mapped to physical or swap space. It is critical to
\emph{coordinate} the mapping of these different virtual resources to ensure that a
thread has all of the resources required at any given time mapped to the
physical space, to enable execution with minimal overhead.

\subsection{Design Overview: Key Ideas}

To solve these challenges, \X employs two key ideas. First, we
leverage software (the compiler) to provide \revision{annotations with
  information} regarding the resource requirements of each phase of
the application. This information enables the framework to make
intelligent decisions dynamically regarding both the extent of
oversubscription and the allocation/deallocation of resources whenever
required.

Second, we use an
adaptive runtime system to actively control the mapping between the
virtual space and the physical space. This control allows us to \emph{(i)} dynamically
alter the number of threads executing to change the extent of
oversubscription at runtime, and \emph{(ii)} continuously coordinate
the mapping between the virtual and physical spaces.
% based on the run time requirements of the
%application. 

\subsubsection{Leveraging Software \revision{Annotations} of Phase
Characteristics}
\label{sec:key_idea_phases}
%The number of registers and the amount of scratchpad used in an application
%tends to vary
%throughout the execution of each thread. 
\ignore{
It is well
known~\cite{compiler-register,virtual-register,gebhart-hierarchical,energy-register} that the
number of live registers changes throughout execution, and since the compiler
allocates registers to hold the worst-case maximum, the number of live
registers at any time is very often far fewer than the number allocated. 
%This happens because the compiler allocate registers to
%hold the worst-case maximum number of live values at any point in the entire
%program~\cite{virtual-register}.
Similarly, scratchpad is typically only
used for a fraction of the total execution of a thread
block, leaving it underutilized for significant
fractions of the execution time~\cite{shmem-multiplexing}. 
}

In addition to the runtime variation in resource
requirement~\cite{compiler-register,virtual-register,gebhart-hierarchical,energy-register}, 
%We observe the same variation in utilization in the workloads in our study, but 
we also observe
that this variation typically occurs at 
%in moderately coarse
granularities or \emph{phases} of a few tens of instructions.
%This coarse-grained variation occurs for a few reasons. First, different
%functions called within the
%kernel tend to have significantly different live register or scratchpad working sets.
This variation occurs because different parts of kernels perform different operations that
require
different resources. For example, loops that simply load/store data to scratchpad
memory use scratchpad but tend to be less register heavy. Sections of code
that perform specific computations (e.g. matrix transformation, graph
manipulation), may either be register heavy or primarily operate out
of scratchpad. Often, scratchpad is used for only short intervals~\cite{shmem-multiplexing}, e.g., when data exchange between threads is
required, such as a reduction
operation.   
\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\textwidth]{figures/Phase_nqu-crop.pdf}
  \caption{Example Phases: NQU. Reproduced from~\cite{zorua}.}
  \label{fig:phases}
\end{figure} 

Figure~\ref{fig:phases} depicts a few example phases from the NQU (\emph{N-Queens Solver}) kernel.
NQU is a scratchpad heavy
application but uses no scratchpad during the initial computation. During the
second phase, it performs its primary computation out of scratchpad and uses as much as
4224B. During the last phase, the
scratchpad is now used only for reducing
results which only requires 384B of
scratchpad. There is also a significant variation in the maximum number of live
registers in the different phases.    
\ignore{
\begin{figure}[h]
  \centering
  \begin{subfigure}[b]{0.99\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/Phase_dct-crop.pdf}
  \caption{DCT}
  \label{fig:phase_dct}
  \end{subfigure} 
  \begin{subfigure}[b]{0.99\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/Phase_nqu-crop.pdf}
  \caption{NQU}
  \label{fig:phase_nqu}
  \end{subfigure}
  \caption{Example Phases. Adapted from~\cite{zorua}.}
  \label{fig:phases}
\end{figure} 

Figure~\ref{fig:phases} depicts two examples kernels: DCT (\emph{Discrete Cosine
Transform}) and NQU (\emph{N-Queens Solver})\footnote{It should be noted that
we do not depict the entire kernel and all of its phases for the sake of brevity. We
merely depict a few example phases from the kernel.}. \new{In DCT
(Figure~\ref{fig:phase_dct}), the first few instructions perform index
computation and load the scratchpad. This phase contains at most 16 live
registers at any time. The function calls that perform the Cosine Transform have
a significantly larger register working set, requiring 32 registers. The
scratchpad is, however, live for most of the execution. }NQU
(Figure~\ref{fig:phase_nqu}), is a scratchpad heavy application. It uses no
scratchpad during the initial computation. During the second phase, the
application performs its primary computation out of the scratchpad and as much as
4224B of scratchpad (the maximum allocated) is used. During the last phase, the
scratchpad is now used only for reducing
results from the previous computation and this reduction only requires 384B of
scratchpad.    
}

In order to capture both the resource requirements as
well as their variations over time, we 
%leverage the (moderately) coarse granularity in variation to 
partition the program into a number of \emph{phases}. A phase is
essentially a sequence of instructions with sufficiently different resource
requirements than adjacent phases. Barrier or fence operations 
also indicate a change in requirement for a different
reason -- threads that are waiting at a barrier do not momentarily require the
thread slot that they are holding. 
%Rather, they require progress of
%\emph{other} threads in the same thread block. 
We interpret
barriers and fences as phase boundaries as they potentially alter the
utilization of their thread slots. Section~\ref{sec:phase_specifiers} contains more details on
the semantics of phases and phase specifiers.  
 
A phase forms the basic unit or \emph{handle} for resource allocation and de-allocation as well
as for making decisions on oversubscription. 
Phases offer a more fine-grained granularity than that of
an entire thread to make oversubscription decisions. The phase specifiers
provide knowledge of the future resource usage of the thread at a phase
boundary. This enables \emph{(i)} preemptively controlling the extent of
oversubscription at runtime, and \emph{(ii)} dynamically allocating and deallocating
resources at phase boundaries to maximize utilization of the physical resources.

\subsubsection{Control with an Adaptive Runtime System}
Phases provide a handle as well as information to make oversubscription and allocation/deallocation
decisions. However, we still need a way to dynamically make decisions on oversubscription
and mapping, and enforce them at runtime. To this end, we use an adaptive
runtime system to dynamically control the mapping between the virtual
and physical spaces.  
We refer to this system as the \emph{coordinator}. Figure~\ref{fig:coordinator}
presents an overview of the functioning of the coordinator.

The virtual space provides an illusion of a flexible amount of
each of the resources to adapt to different application requirements. This illusion enables higher \emph{effective parallelism}
than what can be achieved with simply the fixed physically available resources
by executing many \emph{active threads} concurrently. 
\ignore{However, at run time, the resource requirements of each application changes in
two ways. First, the register file and scratchpad requirements varies depending on the
phase of the application. Second, barriers/fences control the number of threads
actively executing at any time. Any thread waiting at a barrier does not
momentarily require its thread slot -- rather, it requires the execution of
\emph{other} threads in the thread block to proceed in execution. }
However, at runtime, the resource requirements of each application continuously
change. In order to 
adapt to these runtime changes, the coordinator controls the extent of oversubscription by altering the 
number of threads presented to the warp scheduler and compute units. The coordinator
partitions the active threads into \emph{schedulable threads} and \emph{pending
threads}. At any given time, the warp scheduler only views the schedulable
threads that are selected by the coordinator. 

The coordinator leverages information from the phase
specifiers to make decisions on oversubscription at every phase boundary
(detailed in Section~\ref{sec:mechanism}). The coordinator also 
controls and coordinates the mapping between the virtual and physical/swap
space based on the information from the phase specifiers. 

\ignore{\textbf{Summary.} The coordinator employs an additional layer of indirection
between the virtual space and physical space to control the extent of
oversubscription by dynamically altering the number of threads presented to the
warp scheduler. The coordinator uses the hints provided by the phase specifiers
to make the oversubscription decisions and allocate or deallocate resources at
each phase boundary.  
}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{figures/coordinator-crop.pdf}
  \caption{Overview of the Coordinator. Reproduced from~\cite{zorua}.}
  \label{fig:coordinator}
\end{figure} 





%============================oldwriting============================
\ignore{\subsection{Design Summary}
\subsubsection{Controlling the extent of oversubscription}
During every phase change, the phase specifier denotes the resources required
for the next phase. This enables the decision at each
phase change whether scheduling the next phase for execution would fit within the desired
extent for oversubscription. 


\subsubsection{Control and Coordination of mapping}
Phase specifiers enable fine-grained management of resource requirements.
Resources are allocated and de-allocated at the granularity of a phase. Each
phase specifier only allocates those resources required for the execution of the
phase. At the end of a phase, those resources that are no longer required are
explicitly deallocated. 
}

\ignore{Figure X depicts an overview of the proposed framework. To control both the
extent of oversubscription as well as the mapping between virtual and
physical/swap space, we introduce an entity in hardware referred to as the
\emph{coordinator}. Every cycle, the coordinator determines the size of the
virtual space for each of the resources. It also determines the mapping of
different virtual resources to physical and swap spaces. Thread blocks that are scheduled to each SM are
first handed to the coordinator. Based on the determined extent of
oversubscription and mapping, the coordinator determines both how many warps
and which warps to provide to the warp scheduler. Section X contains a more
detailed description of the functioning of the coordinator. The warp
scheduler operates independently of the coordinator potentially employing any
scheduling algorithm.

\subsection{Spatio-Temporal Management with Phases}
In order to capture both the on-chip resource requirements of each thread as
well as its variance over time, we divide the program into a number of \emph{phases}. A phase is
essentially a sequence of instructions with significantly different resource
requirements than the previous or next phase. Every barrier or fence operation
also divides the program into phases.

A phase forms the basic unit for resource allocation and de-allocations as well
as for making decisions on oversubscription. The compiler partitions each
application into a number of phases and inserts instructions referred to as
\emph{phase specifiers} to specify the
beginning of each new phase as well as the number of registers and scratchpad
memory required for each phase. Section X contains a more detailed description
of determining phases from applications. We now discuss the how the key
challenges are addressed using the coordinator and phases. 

\subsubsection{Controlling the extent of oversubscription}
During every phase change, the phase specifier denotes the resources required
for the next phase. The allows the coordinator to make the decision at each
phase change whether scheduling the phase for executions fits within the desired
extent for oversubscription. Phases offer both a more fine-grained granularity than that of
an entire thread to make oversubscription decisions. Also, the phase specifiers
provide knowledge of the future resource usage of the thread at a phase
boundary. This enables the coordinator to preemptively control the extent of
oversubscription and make intelligent decisions.

\subsubsection{Control and Coordination of mapping}
Phase specifiers enables fine-grained management of resource requirements.
Resources are allocated and de-allocated at the granularity of a phase. Each
phase specifier only allocates those resources required for the execution of the
phase. At the end of a phase, those resources that are no longer required are
explicitly deallocated. 

}


\ignore{\thoughts{Discuss at how we address each of the above challenges.}
\thoughts{High-level summary of the solution.}
\subsection{Hardware-based solution with Compiler Hints.}
\thoughts{Justify why a hardware-based solution makes sense.}
\subsection{Spatio-temporal Virtualization with Phases.}
\thoughts{Description of how phases work with an with an example.}
\subsection{Adaptive Dynamic Oversubscription.}
\thoughts{Describe the functioning of the coordinator.}
}


==> sections/goal.tex <==
\section{Goal}

Our goal in this work is to bridge this disparity between the application
requirements and available hardware resources completely \emph{transparent} to
the programmer. In order to address both the spatial and temporal disparity, we propose to introduce another level of indirection between the
application and hardware to effectively \emph{virtualize} the different on-chip
resources. To this end, we develop a framework to \emph{(i)} adapt to the varying
run time requirements of the application and \emph{(ii)} provide an \emph{illusion} of the required resources
to achieve the desired level of parallelism to maximize performance and energy
efficiency for any application. We refer to this framework as \Xfull or \X.

\X comprises two key functionalities to address the two key sources of
inefficiency, i.e., the spatial and temporal disparity. First, \X dynamically
allocates and de-allocates physical resources as and when required depending on
the run-time requirements of the application in order to maximize the
utilization of resources. Second, when there are insufficient available
physical resources, \X still provides the illusion of desired amount of
resources by \emph{oversubscribing} each of the on-chip resources as required.

Figure X depicts the high-level overview of the proposed framework. The
\emph{application space} refers to the required resources at any given time. For
the register file and scratchpad memory, it includes the \emph{live} registers
and scratchpad content at any given time. This application space is serviced by
a the proposed \emph{virtual space}. The virtual space provides an illusion of
the desired amount of each of the three resources and decides the parallelism
for the application at any given time. The \emph{physical space} refers to the
actual hardware resources specific to each architecture and the \emph{swap
space} refers to the resources that belong to the virtual space but do not fit
in the physical space and are hence spilled to the swap space. In the case of
the register file and scratchpad memory, the swap space is mapped to global
memory space, which may be found in the caches or in main memory. In the case of
threads, only those threads are mapped to the physical space are available for
scheduling and execution at any given time. The state (the PC and SIMT stack)
are saved in memory, if the thread is mapped to the swap space. Different
resources in the virtual space, can be freely mapped and re-mapped between the
physical and swap spaces to provide the illusion of the virtual space resources.
 
In
designing such a framework, there are several key challenges which
now describe.
\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\textwidth]{figures/Overview-crop.pdf}
  \caption{High-level Overview of \X}
  \label{fig:overview}
\end{figure} 

%================oldwriting==========================================
\ignore{\begin{itemize}
\item Bridge the disparity between the application and the physical resources
transparent to the programmer -- add another level of indirection.
\item Address both the spatial and temporal disparity by virtualizing the
different on-chip resources.
\end{itemize}
}


